Plant-wide byproduct gas distribution under uncertainty in iron and steel industry via quantile forecasting and robust optimization

In the modern iron and steel industry, the efficient distribution of byproduct gases faces significant challenges due to quantity- and quality-related uncertainties of gases. This study presents an optimal approach to gas distribution that addresses this issue by incorporating the energy flow network and the uncertain surplus gases from the manufacturing system. The uncertain optimization problem is formulated as a two-stage robust optimization (TSRO) model, including "here-and-now" decisions aimed at minimizing the start-stop cost of energy conversion units, as well as "wait-and-see" decisions aimed at minimizing the operating cost of gasholders and the penalties resulting from energy excess or shortage. To facilitate practical implementation, we propose a "first quantify, then optimize" approach: (1) quantifying the uncertainty of surplus gases via a conditional quantile regression (CDQ)-based T-step time series model, and (2)finding the optimal solution through a column-and-constraint generation algorithm. Furthermore, a case study is conducted on an industrial energy system to validate the proposed methodology. Computational results, using evaluation indicators, such as MAPE, RMSE, PICP, and PINAW, confirm the effectiveness of the data-driven time series model in accurately quantifying uncertainties in each period. Sensitivity analysis demonstrates that the proposed TSRO model achieves a favorable balance between robustness and flexibility by selecting the combination of "budget and quantile" and the parameters of storage and conversion units. Consequently, TSRO can efficiently find a robust gas distribution solution with the desired level of conservativeness for integrated iron and steel plants.

==> Notations.tex <==
\nomenclature[D01]{$\mathcal{K},k$}{Vertex in the energy network}
\nomenclature[D02]{$\mathcal{A},a$}{Arcs in the energy network}
\nomenclature[D03]{$\mathcal{G},g$}{Energy in the energy network}
\nomenclature[D04]{$\mathcal{T},t$}{Time periods of energy distribution}

\nomenclature[P01]{$\mathcal{A}^{+}(k)$, $\mathcal{A}^{-}(k)$ }{Input and output arcs of vertex $k$}
\nomenclature[P02]{${a}^{+}$, ${a}^{-}$ }{Origin and destination vertex of arc $a$}
\nomenclature[P03]{$e:a$}{Energy of arc $a$}
\nomenclature[P04]{$\omega_{a}$}{Calorie value of the energy flow on arc $a$}
\nomenclature[P05]{$\rho_{k}$}{conversion efficiency of energy unit on vertex $k$}
\nomenclature[P06]{$z_{a,t}$}{Suplus gas at time pertiod $t$}
\nomenclature[P07]{$d_{a,t}$}{Demand of energy eat time pertiod $t$}
\nomenclature[P08]{$\eta_{k}^+$}{Minimum calorie value of the input energies to conversion unit $k$}
\nomenclature[P09]{$\eta_{k}^-$}{Minimum ratio of the ouput energies from conversion unit $k$ to their maximum flows}
\nomenclature[P10]{$\overline{U}_{k}$}{Maximum volume of gasholder $k$}
\nomenclature[P11]{$\underline{U}_{k}$}{Minimum volume of gasholder $k$}
\nomenclature[P12]{$\Delta_{k}$}{Minimum devivation of gasholder $k$}		
\nomenclature[P13]{$\overline{F}^{+}_{k,a}$}{Maximum flow of input energy $a$ of conversion unit $k$}
\nomenclature[P14]{$\underline{F}^{+}_{k,a}$}{Minimum flow of input energy $a$ of conversion unit $k$}	
\nomenclature[P15]{$\overline{F}^{-}_{k,a}$}{Maximum flow of output energy $a$ of conversion unit $k$}
\nomenclature[P16]{$\underline{F}^{-}_{k,a}$}{Maximum flow of output energy $a$ of conversion unit $k$}
\nomenclature[P17]{$\gamma_1$}{Objective coefficient of the start-stop costs}
\nomenclature[P17]{$\gamma_2$}{Objective coefficient of the gasholders operating costs}
\nomenclature[P18]{$\gamma_{3,k}$}{Objective coefficient of surplus and shorages of demand $k$}	

\nomenclature[V1]{$f_{a,t}$}{Continuous variable, which represents the flow of arc $a$ at time period $t$ }
\nomenclature[V2]{$u_{k,t}$}{Continuous variable, which represents stroaage level of unit $v$ at time period $t$ }
\nomenclature[V3]{$v_{g,t}$}{Continuous variable, which represents shortage or over-stock of energy $e$ at time period $t$ }
\nomenclature[V4]{$O_{k,t}$}{Binary variable, which represents the running state (on and off) of conversion unit $k$  at time period $t$}
\nomenclature[V5]{$S_{k,t}$}{Binary variable, which represents the switch state (start up and shut down) of conversion unit $k$  at time period $t$}

\printnomenclature


